Observation of $\Lambda_{b}^{0} \to \Lambda_{c}^{+} \bar{D}^{(*)0} K^{-}$ and $\Lambda_{b}^{0} \to \Lambda_{c}^{+} D_{s}^{*-}$ decays

The decays $\Lambda_b^0 \to \Lambda_c^+\bar{D}^{(*)0}K^-$ and $\Lambda_b^0 \to \Lambda_c^+ D_s^{*-}$ are observed for the first time, in proton-proton collision data at $\sqrt{s}=13$TeV corresponding to an integrated luminosity of 5.4 fb${}^{-1}$ collected with the LHCb detector. Their ratios of branching fractions with respect to the $\Lambda_b^0\!\to\Lambda_c^+\mathrm{D}_s^-$ mode are measured to be \begin{align*} \begin{split} \frac{\mathcal{B}(\Lambda_b^0 \to \Lambda_c^+\bar{D}^0 K^-)}{\mathcal{B}(\Lambda_b^0 \to \Lambda_c^+ D_s^-)} & = 0.1908 {}_{-0.0034}^{+0.0036} {}_{-0.0018}^{+0.0016} \pm 0.0038 \frac{\mathcal{B}(\Lambda_b^0 \to \Lambda_c^+\bar{D}^{*0} K^-)}{\mathcal{B}(\Lambda_b^0 \to \Lambda_c^+ D_s^-)} & = 0.589 {}_{-0.017}^{+0.018} {}_{-0.018}^{+0.017} \pm 0.012 \frac{\mathcal{B}(\Lambda_b^0 \to \Lambda_c^+ D_s^{*-})}{\mathcal{B}(\Lambda_b^0 \to \Lambda_c^+ D_s^-)} & = 1.668 \pm 0.022 {}_{-0.055}^{+0.061}\ , \end{split} \end{align*} where the first uncertainties are statistical, the second systematic, and the third, for the $\Lambda_b^0 \to \Lambda_c^+ \bar{D}^{(*)0} K^-$ decays, are due to the uncertainties on the branching fractions of the $D_s^- \to K^- K^+ \pi^-$ and $\bar{D}^0 \to K^+\pi^-$ decay modes. The measured branching fractions probe factorization assumptions in effective theories and provide the normalization for future pentaquark searches in $\Lambda_b^0 \to \Lambda_c^+ \bar{D}^{(*)0}K^-$ decay channels.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)



==> tables/LbToLcDssmRun2_selA_fitA_unfA_multA_wtypA_wsetA_dfromb_hi.tex <==
0.0

==> tables/LbToLcDssmRun2_selA_fitA_unfA_multA_wtypA_wsetA_dfromb_lo.tex <==
0.0

==> tables/LbToLcDssmRun2_selA_fitA_unfA_multA_wtypA_wsetA_wo_dbf.tex <==
1.668 \pm 0.022 {}_{-0.055}^{+0.061}

==> tables/LbToLcDstarzbKmRun2_selA_fitA_unfA_multA_wtypA_wsetA_dfromb_hi.tex <==
0.1

==> tables/LbToLcDstarzbKmRun2_selA_fitA_unfA_multA_wtypA_wsetA_dfromb_lo.tex <==
0.1

==> tables/LbToLcDzbKmRun2_selA_fitA_unfA_multA_wtypA_wsetA_dfromb_hi.tex <==
0.1

==> tables/LbToLcDzbKmRun2_selA_fitA_unfA_multA_wtypA_wsetA_dfromb_lo.tex <==
0.1

==> tables/LbToLcDzbKmRun2_selA_fitA_unfA_multA_wtypA_wsetA_total_lo.tex <==
0.9
